Rethinking Hallucinations: Correctness, Consistency, and Prompt Multiplicity

Large language models (LLMs) are known to "hallucinate" by generating false or misleading outputs. Hallucinations pose various harms, from erosion of trust to widespread misinformation. Existing hallucination evaluation, however, focuses only on correctness and often overlooks consistency, necessary to distinguish and address these harms. To bridge this gap, we introduce prompt multiplicity, a framework for quantifying consistency in LLM evaluations. Our analysis reveals significant multiplicity (over 50% inconsistency in benchmarks like Med-HALT), suggesting that hallucination-related harms have been severely misunderstood. Furthermore, we study the role of consistency in hallucination detection and mitigation. We find that: (a) detection techniques detect consistency, not correctness, and (b) mitigation techniques like RAG, while beneficial, can introduce additional inconsistencies. By integrating prompt multiplicity into hallucination evaluation, we provide an improved framework of potential harms and uncover critical limitations in current detection and mitigation strategies.

==> sections/background.tex <==
\section{Experiment setup}
\label{sec:background}

% \subsection{LLM Hallucinations Taxonomy}

% \prakhar{The whole subsection is not really needed. Move parts of it to appropriate locations and remove it from here.}

% The term ``hallucinations'' has evolved significantly over the years, shifting from a positive connotation in computer vision~\citep{baker2000hallucinating,hsu2010face} to its current association with generating nonsensical text in NLP~\citep{blog2015unreasonable,huang2023survey,ji2023survey,zhang2023siren}. While the term has been debated--often replaced by alternatives like `fabrication' or `confabulation'~\citep{venkit2024audit}--it remains widely accepted in the community. For consistency, we also stick with the term hallucinations when referring to previous literature. However, an important objective of our work is to rethink the true harms of generating false, nonsensical, or unfaithful content, particularly in the context of their stability. To that end, we will incorporate other relevant terminologies from the literature where appropriate.

% An important framework that we draw upon comes from knowledge extraction in LLMs~\citep{jiang2020can,zhu2024llms}. Recent work by \citet{yin-etal-2024-benchmarking} introduced \textit{prompt-agnostic knowledge}--that can be extracted using most prompts--and \textit{prompt-sensitive knowledge}--that can only be retrieved with specific prompts. A similar distinction is needed in LLM hallucinations, and we adopt this taxonomy in our analysis.

% \subsection{Datasets, Models, and Paraphrasing}
% \prakhar{This will become a complete section. Make edits and add more details accordingly.}

\golnoosh{You need to provide some context here for the reader. It is very sudden to talk about the experiment setup. I suggest moving it to 4.2 after defining decision multiplicity. }
\paragraph{Datasets.} 

We will use the following benchmarks in our paper: Wiki-FACTOR dataset from FACTOR~\citep{muhlgay2024generating}, Reasoning Hallucination Test (RHT) from Med-HALT~\citep{pal2023med}, MCQ task from TruthfulQA~\citep{lin2022truthfulqa}, all topics combined from True-False~\citep{azaria2023internal}, development set of CommonsenseQA~\citep{talmor2019commonsenseqa}, and shared task development set of FEVER~\citep{thorne2018fever}. More details on each dataset and their evaluation setup are provided in the appendix (\S \ref{sec:app_datasets}). We will use TruthfulQA, Wiki-FACTOR, and Med-HALT for the main paper, while additional results for other benchmarks are delegated to the appendix.

We limit our study to MCQ settings and use the perplexity-based evaluation by \citet{muhlgay2024generating} for all benchmarks. We chose MCQ-style benchmarks because other benchmarks that allow freeform generation require an additional automated method to compare generated outputs against the gold truth or detect hallucinations in the text. In most cases, such benchmarks rely on LLMs as judges~\citep{lin2022truthfulqa,li2023halueval,dong2024bamboo}--which can introduce its own errors, biases, and multiplicity~\citep{li2024generation,ye2024justice,panickssery2024llm}. Thus, we stick with MCQ-style benchmarks to maintain a clear focus on multiplicity in LLM hallucinations. Moreover, our study is limited to factuality hallucinations, due to their popularity~\citep{li2024dawn}.

\paragraph{Models.} 

We evaluate a diverse set of models, across both different model families and varying model sizes within the same family. Specifically, we use the following models: GPT-J-6B~\citep{gptj}, GPT-NeoX-20B~\citep{black2022gpt}, Pythia-2.8B/6.9B/12B~\citep{biderman2023pythia}, Bloom-3B/7.1B~\citep{workshop2022bloom}, Llama2-7B/7B-Chat/13B/13B-Chat~\citep{touvron2023llama}, Llama3-8B/8B-Instruct~\citep{dubey2024llama}, and OPT-6.7B/13B/30B~\citep{zhang2022opt}. 
% While the key experiments are conducted on all models, we avoid extremely large models like 70B Llama variants for most ablation studies.

\paragraph{Prompt Variations and Paraphrasing.} 

Five out of the six benchmarks in our paper are evaluated with demonstrations in the prompt. Thus, we simulate prompt variations by shuffling the order of demonstrations~\citep{lu2022fantastically}, as these adjustments can be controlled and applied consistently across the dataset. However, for the Wiki-FACTOR dataset, we have to turn to automated paraphrasing, for which we use a fine-tuned T5 model~\citep{raffel2020exploring} trained on a paraphrase dataset from ChatGPT~\citep{chatgpt_paraphraser, chatgpt_paraphrases_dataset}. We leave the in-depth exploration of various forms of prompt variations and their individual impact on LLM hallucinations for future work.



% \subsection{Datasets}

% There are several LLM hallucination datasets, growing rapidly every day. A useful culmination of this is the open source efforts by \citet{hong2024hallucinations} to create a unified benchmark that measures performance over a large set of datasets.

% However, for our experiments, we are going to look at a more granular level of individual datasets and sentences. We have currently experimented with the following datasets,

% \paragraph{LAMA} LAMA~\citep{petroni2019language} dataset is a collection of facts from various websites, stored in a structured form. For example, a task in the LAMA dataset is country and capital, where the names of the country and their capital are stored in a structured format. During evaluation, a template is used, such as, \textit{The capital of [X] is [Y]}, and appropriate names are filled into the template to check for hallucinations. This is a great dataset for very granular control over evaluations, but since it only evaluates the generation of 1-2 words at most, it doesn't capture the true range of LLM hallucinations.

% \paragraph{TruthfulQA} TruthfulQA~\citep{lin2022truthfulqa} dataset contains around half of its data designed manually by experts to represent common misconceptions that are held by humans, and the other half of its data designed together with a language model to do the same thing, but this time the options are created using the language model. It contains questions like, 'What would happen if you burn the UK flag in the UK?', and while some humans might have misconceptions of there being a law against it, there isn't one. This dataset aims to capture such misconceptions and see if they are reflected in LLMs too. The dataset, however, contains several issues, including problems like many questions containing 'No comment' as the correct answer (which the LLM isn't likely to prefer).

% \paragraph{FACTOR} FACTOR~\citep{muhlgay2024generating} dataset is created by first extracting sentences from a certain knowledge base (like Wikipedia), followed by using InstructGPT to create false completions of that sentence given the correct completion. These false completions are small perturbations (1-2 words) on the original completion such that it changes the meaning of the sentence. For example, the word 'positive' might be replaced with the word 'negative', or if there is a date present in the sentence, that date would be changed to some other random date, etc. FACTOR is a significant improvement over TruthfulQA in terms of quality, however, the facts contained in FACTOR might resemble 'memorization' more than true factual knowledge.

% \paragraph{HaluEval} HaluEval~\citep{li2023halueval} dataset is a good improvement over both TruthfulQA and FACTOR datasets. It contains reasonable facts and not just general Wikipedia sentences like in FACTOR. At the same time, it also contains good continuations and not just continuations like 'No comment' in TruthfulQA. However, the evaluation technique suggested by their paper for HaluEval is quite unintuitive. Instead of treating it as a multiple-choice task, they suggest 'randomly' choosing an option and then asking the LLM in a natural language form whether the chosen option is a hallucination or not.

% \subsection{Pythia}

% Pythia~\citep{biderman2023pythia} is a suite of LLM models trained on the Pile dataset for various model sizes. What sets these models apart is that each model in their suite is trained on the same fixed data order, which is available with the models for anyone to study and replicate. Each model in the suite has 154 checkpoints, 144 of them being equally spaced throughout the entire training process, while the remaining 10 are exponentially spaced at the start of training. This allows us to observe how the model evolves as it trains on more and more data. We have access to both the model checkpoints and the exact data seen by the model in this process, enabling us to inspect the impact of data order.

% Pythia has also conducted preliminary experiments that indirectly test how the order of data affects the behaviour of LLM models~\citep{biderman2024emergent}. One of their experiment measured how well the training data was memorized and found that the position of the data point in the order didn't affect its chances of being memorized. Another experiment focused on bias mitigation techniques applied to data in only the last few iterations of model training. They discovered that applying bias mitigation to only the last 7\% of the overall data led to significant improvements in fairness. Moreover, extending this to the last 21\% of the data didn't amplify the impact much more.
